Some aspects of descent theory and applications

This thesis is an exposition of the author's contribution on effective descent morphisms in various categories of generalized categorical structures. It consists of: Chapter 1, where an elementary description of descent theory and the content of each remaining chapter is provided, supplemented with references; Chapter 2, consisting of various descent theoretical definitions and results employed in the remainder of this work; four chapters, each corresponding to an article written by the author during the period of his PhD studies.

==> preamble.tex <==
% ******************************************************************************
% ****************************** Custom Margin *********************************

% Add `custommargin' in the document class options to use this section
% Set {innerside margin / outerside margin / topmargin / bottom margin}  and
% other page dimensions
\ifsetCustomMargin
  \RequirePackage[left=28mm,right=28mm,top=35mm,bottom=30mm]{geometry}
  \setFancyHdr % To apply fancy header after geometry package is loaded
\fi

% *****************************************************************************
% ******************* Fonts (like different typewriter fonts etc.)*************

% Add `customfont' in the document class option to use this section

\ifsetCustomFont
  % Set your custom font here and use `customfont' in options. Leave empty to
  % load computer modern font (default LaTeX font).
  \RequirePackage{helvet}
\fi

% *****************************************************************************
% ******************* COVER / CAPA ********************************************
\usepackage{pdfpages}

% *****************************************************************************
% **************************** Custom Packages ********************************

\usepackage[all]{xypic}
\usepackage{tikz-cd}
\usepackage{amsthm}
\usepackage{enumitem}
\usepackage[utf8]{inputenc}
%\usepackage{algpseudocode}


% ********************Captions and Hyperreferencing / URL **********************

% Captions: This makes captions of figures use a boldfaced small font.
%\RequirePackage[small,bf]{caption}

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty


% *************************** Graphics and figures *****************************

%\usepackage{rotating}
%\usepackage{wrapfig}

% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
\usepackage{subcaption}

% ********************************** Tables ************************************
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}


% ***************************** Math ******************************

\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}


% ******************************* Line Spacing *********************************

% Choose linespacing as appropriate. Default is one-half line spacing

% \doublespacing
% \onehalfspacing
% \singlespacing


% ************************ Formatting / Footnote *******************************

% Don't break enumeration (etc.) across pages in an ugly manner (default 10000)
%\clubpenalty=500
%\widowpenalty=500

%\usepackage[perpage]{footmisc} %Range of footnote options


% *****************************************************************************
% *************************** Bibliography  and References ********************

%\usepackage{cleveref} %Referencing without need to explicitly state fig /table

% Add `custombib' in the document class option to use this section
%   \RequirePackage[square, sort, numbers, authoryear]{natbib} % CustomBib

% If you would like to use biblatex for your reference management, as opposed
   % to the default `natbibpackage` pass the option `custombib` in the
   % document class. Comment out the previous line to make sure you don't load
   % the natbib package. Uncomment the following lines and specify the
   % location of references.bib file

\usepackage[backend=biber,
                style=trad-plain,
                citestyle=numeric,
                sorting=nty]{biblatex}
            
\DefineBibliographyStrings{english}{%
  page             = {p.},
  pages            = {pp.},
} 

\addbibresource{references.bib} %Location of references.bib only for biblatex


% changes the default name `Bibliography` -> `References'
%\renewcommand{\bibname}{References}


% ********************** TOC depth and numbering depth *************************

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


% ******************************* Nomenclature *********************************

% To change the name of the Nomenclature section, uncomment the following line

%\renewcommand{\nomname}{List of Symbols}


% ********************************* Appendix ***********************************

% The default value of both \appendixtocname and \appendixpagename is `Appendices'. These names can all be changed via:

%\renewcommand{\appendixtocname}{List of appendices}
%\renewcommand{\appendixname}{Appndx}

% ******************************** Draft Mode **********************************

% Uncomment to disable figures in `draftmode'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


%% Todo notes functionality
%% Uncomment the following lines to have todonotes.

%\ifsetDraft
%	\usepackage[colorinlistoftodos]{todonotes}
%	\newcommand{\mynote}[1]{\todo[author=kks32,size=\small,inline,color=green!40]{#1}}
%\else
%	\newcommand{\mynote}[1]{}
%	\newcommand{\listoftodos}{}
%\fi

% Example todo: \mynote{Hey! I have a note}

% ========================================================================== %
% Shortcut commands/notation
% ========================================================================== %

% Fixed letters

\newcommand{\op}{\mathsf{op}}
\newcommand{\R}{\mathbb R}
\newcommand{\N}{\mathbb N}

\renewcommand{\epsilon}{\varepsilon}
\newcommand{\id}{\mathsf{id}}
\newcommand{\ev}{\mathsf{ev}}
\newcommand{\lax}{\mathsf{lax}}
\newcommand{\lc}{\ell} % Placeholder
\newcommand{\opl}{\mathsf{opl}}
\newcommand{\fin}{\mathsf{fin}}
\newcommand{\str}{\mathsf{str}}
\newcommand{\conn}{\mathsf{conn}}
\newcommand{\heps}{\hat{\epsilon}}
\newcommand{\hups}{\hat{\upsilon}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\heta}{\hat{\eta}}


\renewcommand{\emptyset}{\varnothing}
\newcommand{\Rho}{\text{P}}
\newcommand{\Alpha}{\text{A}}

\newcommand{\lng}{\langle}
\newcommand{\rng}{\rangle}

\newcommand{\comma}{\downarrow}
\newcommand{\cat}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\intcat}[1]{\ensuremath{\mathscr{#1}}}
\newcommand{\bicat}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\ovln}[1]{\ensuremath{\overline{#1}}}

\newcommand{\dash}{\text{-}}

% Names of categories 
\newcommand{\catname}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\Set}{\catname{Set}}
\newcommand{\Cat}{\catname{Cat}}
\newcommand{\Stn}{\catname{Stn}}
\newcommand{\CHaus}{\catname{CHaus}}
\newcommand{\MultiCat}{\catname{MultiCat}}
\newcommand{\VMultiCat}{\cat V \dash \MultiCat}
\newcommand{\Grph}{\catname{Grph}}
\newcommand{\RGrph}{\catname{RGrph}}
\newcommand{\Bicat}{\catname{Bicat}}
\newcommand{\CatV}{\Cat(\cat V)}
\newcommand{\VCat}{\cat V\dash\Cat}
\newcommand{\Mod}{\catname{Mod}}
\newcommand{\ModSV}{\Mod(\cat S,\cat V)}
\newcommand{\CAT}{\catname{CAT}}
\newcommand{\VCAT}{\cat V \dash\CAT}
\newcommand{\DbCat}{\catname{DbCat}}
\newcommand{\PsDbCat}{\catname{PsDbCat}}
\newcommand{\SymCat}{\catname{SymCat}}
\newcommand{\Lax}{\catname{Lax}}
\newcommand{\Ps}{\catname{Ps}}
\newcommand{\Mnd}{\catname{Mnd}}
\newcommand{\Alg}{\catname{Alg}}
\newcommand{\Mat}{\catname{Mat}}
\newcommand{\Span}{\catname{Span}}
\newcommand{\SpanV}{\Span(\cat V)}
\newcommand{\VMat}{\cat V\dash \Mat}
\newcommand{\SpanB}{\Span(\cat B)}
\newcommand{\LaxTAlg}{T\dash\Lax\Alg}
\newcommand{\LaxidAlg}{\id\dash\Lax\Alg}
\newcommand{\PsTAlg}{T\dash\Ps\Alg}
\newcommand{\Top}{\catname{Top}}
\newcommand{\FamV}{\Fam(\cat V)}
\newcommand{\FamW}{\Fam(\cat W)}
\newcommand{\FamVCat}{\FamV\dash\Cat}
\newcommand{\CatFamV}{\Cat(\FamV)}
\newcommand{\RGrphTV}{\RGrph(T,\cat V)}
\newcommand{\CatTV}{\Cat(T,\cat V)}
\newcommand{\TVCat}{(T, \cat V)\dash\Cat}
\newcommand{\Tt}{\overline T}
\newcommand{\Ff}{\overline F}
\newcommand{\TtVCat}{(\Tt, \cat V)\dash\Cat}
\newcommand{\Desc}{\catname{Desc}}
\newcommand{\Vect}{\catname{Vect}}
\newcommand{\CoDesc}{\catname{CoDesc}}
\newcommand{\FamB}{\Fam(\cat B)}
\newcommand{\FamC}{\Fam(\cat C)}
\newcommand{\FinFam}{\Fam_\fin}
\newcommand{\Equip}{\catname{Equip}}


\newcommand{\RMod}{R\dash\Mod}
\newcommand{\SMod}{S\dash\Mod}

\newcommand{\dsc}{\catname{dsc}}
\newcommand{\indsc}{\catname{indsc}}

\newcommand{\iso}{\cong}
\renewcommand{\leq}{\leqslant}
\newcommand{\eqv}{\simeq}
\newcommand{\sub}{\subseteq}
\newcommand{\adj}{\dashv}

\newcommand{\meet}{\wedge}
\newcommand{\Meet}{\bigwedge}
\newcommand{\join}{\vee}
\renewcommand{\Join}{\bigvee}
\newcommand{\pow}{\pitchfork}

\newcommand{\pt}{\boldsymbol{\cdot}}

\let\lim\relax
\DeclareMathOperator{\Cauchy}{\mathfrak{C}}
\DeclareMathOperator{\ob}{\mathsf{ob}}
\DeclareMathOperator{\dom}{\mathsf{dom}}
\DeclareMathOperator{\cod}{\mathsf{cod}}
\DeclareMathOperator{\lim}{\mathsf{lim}}
\DeclareMathOperator{\colim}{\mathsf{colim}}
\DeclareMathOperator{\Fam}{\catname{Fam}}
\DeclareMathOperator{\Ker}{\catname{Ker}}
\DeclareMathOperator{\Lan}{\catname{Lan}}
\DeclareMathOperator{\Ran}{\catname{Ran}}
\DeclareMathOperator{\Eq}{\catname{Eq}}
\DeclareMathOperator{\Sq}{\catname{Sq}}
\DeclareMathOperator{\PsEq}{\catname{PsEq}}

\DeclareMathOperator{\mult}{\mathsf{m}}
\DeclareMathOperator{\unit}{\mathsf{e}}
\DeclareMathOperator{\idnt}{\mathsf{u}}
\DeclareMathOperator{\comp}{\mathsf{c}}
\DeclareMathOperator{\nat}{\mathsf{n}}
\newcommand{\m}[1]{\mult^{#1}}
\newcommand{\un}[1]{\unit^{#1}}
\newcommand{\cp}[1]{\comp^{#1}}
\newcommand{\tm}[1]{{\tilde\mult}^{#1}}
\newcommand{\e}[1]{\unit^{#1}}
\newcommand{\n}[1]{\nat^{#1}}
\newcommand{\tn}[1]{{\tilde\nat}^{#1}}

\newcommand{\vm}[1]{\m{#1}_v}
\newcommand{\hm}[1]{\m{#1}_h}
\newcommand{\ve}[1]{\e{#1}_v}
\newcommand{\he}[1]{\e{#1}_h}

% ========================================================================= %
% Theorem-like environments
% ========================================================================= %

\newtheorem{lemma}{Lemma}[chapter]
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{corollary}[lemma]{Corollary}

\theoremstyle{definition}
\newtheorem{remark}[lemma]{Remark}

